Accurate calculations of the WIMP halo around the Sun and prospects for gamma ray detection

Weakly interacting massive particles (WIMPs) can be captured by heavenly objects, like the Sun. Under the process of being captured by the Sun, they will build up a population of WIMPs around it, that will eventually sink to the core of the Sun. It has been argued with simpler estimates before that this halo of WIMPs around the Sun could be a strong enough gamma ray source to be a detectable signature for WIMP dark matter. We here revisit the problem using detailed Monte Carlo simulations and detailed composition and structure information about the Sun to estimate the size of the gamma ray flux. Compared to earlier estimates, we find that the gamma ray flux from WIMP annihilations in the Sun halo would be negligible and no current or planned detectors would even be able to detect this flux.

==> fluxtable.tex <==
\begin{table}[ht]
\centering % used for centering table
\begin{tabular}{|c|ccc|r|}
	\hline
$ $ &  $M=100$ GeV    &   $M=1$ TeV  & $M=10$ TeV \\
	\hline
$\sigma_{sd}=10^{-3}$ pb, $\sigma_{si}=0$  & $4.0\cdot 10^{-19}$  & $3.7\cdot 10^{-21}$ & $3.5\cdot 10^{-23}$ \\
$\sigma_{sd}=0$, $\sigma_{si}=10^{-5}$ pb & $8.4\cdot 10^{-20}$  & $2.5\cdot 10^{-21}$ & $2.9\cdot 10^{-23}$ \\
	\hline
\end{tabular}
\caption{The total flux (photons per $\mbox{m}^2$ per second) at Earth of gamma rays from the Sun's WIMP halo.}
\label{table:flux}
\end{table}

